A Survey on RAG Meeting LLMs: Towards Retrieval-Augmented Large Language Models

As one of the most advanced techniques in AI, Retrieval-Augmented Generation (RAG) can offer reliable and up-to-date external knowledge, providing huge convenience for numerous tasks. Particularly in the era of AI-Generated Content (AIGC), the powerful capacity of retrieval in providing additional knowledge enables RAG to assist existing generative AI in producing high-quality outputs. Recently, Large Language Models (LLMs) have demonstrated revolutionary abilities in language understanding and generation, while still facing inherent limitations, such as hallucinations and out-of-date internal knowledge. Given the powerful abilities of RAG in providing the latest and helpful auxiliary information, Retrieval-Augmented Large Language Models (RA-LLMs) have emerged to harness external and authoritative knowledge bases, rather than solely relying on the model's internal knowledge, to augment the generation quality of LLMs. In this survey, we comprehensively review existing research studies in RA-LLMs, covering three primary technical perspectives: architectures, training strategies, and applications. As the preliminary knowledge, we briefly introduce the foundations and recent advances of LLMs. Then, to illustrate the practical significance of RAG for LLMs, we systematically review mainstream relevant work by their architectures, training strategies, and application areas, detailing specifically the challenges of each and the corresponding capabilities of RA-LLMs. Finally, to deliver deeper insights, we discuss current limitations and several promising directions for future research. Updated information about this survey can be found at https://advanced-recommender-systems.github.io/RAG-Meets-LLMs/

==> RAG/Introduction_old.tex <==
\section{Introduction}
\subsection{Large Language/Generative Models}
Recent advances of Generative Artificial Intelligence (GAI) have shown revolutionary abilities in understanding and generating multi-modal content~\cite{lu2024computing}. Large Language Models (LLMs), as a major part of GAI, have made remarkable progress in recent years, with the state-of-the-art models, e.g., GPT series, Gemini~\cite{team2023gemini}, being strongly capable to solve various Natural Language Processing (NLP) and other relevant tasks~\cite{zhao2023survey,achiam2023gpt}. Meanwhile, vision and multi-modal generative models~\cite{podell2023sdxl,driess2023palm} have demonstrated the capability of large pre-trained models for multi-formation content generation. 

Despite of the powerful ability of large generative models, they are still struggling with some inherent limitations and practical challenges~\cite{}, which may lead to unreliable generation or undesirable performance. For example, hallucination is a common issue of LLMs, which describes the phenomenon where the model generates content that are unrealistic, nonsensical or disconnected from the input prompt or context. It can happen especially when queries extend beyond the model's training data or necessitate up-to-date information~\cite{zhang2023siren}. In fact, out-of-scope data and knowledge are major challenges to LLMs due to the essence that they are trained on large amount but fixed-size and biased data, and pre-trained mainly for general-domain tasks. One promising solution to compensate these weaknesses of LLMs is Retrieval-Augmented Generation (RAG)~\cite{lewis2020retrieval}. 

The idea of RAG is to tap into external and authoritative knowledge bases rather than relying on potentially outdated training data or the model's internal knowledge only~\cite{tonmoy2024comprehensive}. Development of large-scale models has demonstrated the beneficial of increasing the size of parameters and enlarging models, which greatly enhance the memorization of the training data but also increase computations significantly. In stead of increasing the model size and training on more data, RAG efficiently augment generation models by equipping them with the ability to directly access additional database to perform prediction~\cite{borgeaud2022improving}. It also provides a way to capture knowledge in a more interpretable and modular way since the knowledge of large generation models is generally considered stored in their parameters, which can only be used implicitly~\cite{guu2020retrieval}. 

RAG was officially introduced by Lewis et al.~\cite{lewis2020retrieval} officially, trying to enhance parametric language generation models with non-parametric memory incorporation, while such idea of boosting generation with retrieval or external knowledge has been applied in many previous work~\cite{chen2017reading,dinan2018wizard,dunn2017searchqa}. As early RAG work, REALM~\cite{guu2020retrieval} and ORQA~\cite{lee2019latent} introduced models combining masked language models (MLM)~\cite{devlin2018bert} with a differentiable retriever. Both the generation and retrieval parts were optimized through large-scale pre-training, which achieved promising results. In comparison, RAG~\cite{lewis2020retrieval} combined a pre-trained generation (BART~\cite{lewis2019bart}) with a retriever (DPR~\cite{karpukhin2020dense}), which is also pre-trained. The retriever and generator are jointly fine-tuned end-to-end through minimizing the negative marginal log-likelihood of the generation results. 

\begin{itemize}
    \item Large Language/Generation Models
    \item External Knowledge/Information Retrieval for LLM
    \item The idea of RAG, what is RGA
    \item capability of RAG
    \item development of RAG
    \item Current status of RAG \& necessity to summarize in this survey
    
\end{itemize}


==> draft.tex <==
\section{Introduction}
\subsection{Existing RAG-relevant surveys}
\begin{itemize}
    \item Retrieval-augmented generation for large language models: A survey~\cite{gao2023retrieval}
    \item Development and Testing of Retrieval Augmented Generation in Large Language Models - A Case Study Report~\cite{ke2024development}
    \item The Chronicles of RAG: The Retriever, the Chunk and the Generator~\cite{finardi2024chronicles}
    \item Retrieval-Augmented Generation for AI-Generated Content: A Survey~\cite{}
    \item A Survey on Retrieval-Augmented Text Generation~\cite{li2022survey}
    \item Retrieving Multimodal Information for Augmented Generation: A Survey~\cite{zhao2023retrieving}
    \item Large language models for information retrieval: A survey~\cite{zhu2023large}
\end{itemize}

\subsection{Possible angles to make another RAG survey}
\begin{itemize}
    \item RAG for hallucination mitigation in large foundation models
    \item RAG techniques and applications
\end{itemize}




\subsection{What is RAG?}
RAG was introduced by Lewis et al. at 2020~\cite{lewis2020retrieval} (claimed by \cite{gao2023retrieval} and \cite{zeng2024good})


\subsection{Why do we need RAG?}
What is large foundation model? How are they applied?
what are limitations of large foundation models? 
\begin{itemize}
    \item hallucination~\cite{zhang2023siren}, especially when queries extend beyond the model's training data or necessitate up-to-date information. Notable techniques to mitigate hallucination in LLMs~\cite{tonmoy2024comprehensive} are RAG, Knowledge Retreival~\cite{varshney2023stitch}, CoNLI~\cite{lei2023chain} and CoVe~\cite{dhuliawala2023chain}, enhancing the model’s utilization of internal knowledge~\cite{liang2024learning}
    \item domain-specific or highly specialized queries~\cite{kandpal2023large} (these two are claimed in \cite{gao2023retrieval})
\end{itemize}
how can RAG address or help with these limitations/drawbacks?
RAG is extensively used to supply LLMs with updated, relevant knowledge, significantly mitigating hallucination~\cite{wu2023ragtruth, gao2023retrieval,gao2023enabling}.

\subsection{Development of RAG?}
\cite{ke2024development}


\subsection{What different RAGs are there? }
Naive RAG, the Advanced RAG, and the Modular RAG~\cite{gao2023retrieval}. 

MultiHop-RAG~\cite{tang2024multihop}

\subsection{RAG for different applications}
Retrieval-Augmented Generation (RAG) has emerged as the most prominent framework for building LLM-based applications. While building a RAG is relatively straightforward, making it robust and a reliable application requires extensive customization and relatively deep knowledge of the application domain.~\cite{fatehkia2024t}

RAG for Electronic Health Records Analysis~\cite{zhu2024realm}

RAG in Finance~\cite{kang2023deficiency}


% \cite{fatehkia2024t} proposed Tree-RAG (T-RAG) to generate a textual description to augment the context when responding to user queries pertaining to entities within the organization's hierarchy. 
RAG for structured textural description generation~\cite{fatehkia2024t}

RAG for QA System~\cite{alan2024rag}
RAG for API call writing~\cite{patil2023gorilla}: Gorilla is a fine-tuned LLaMA-based model with document retriever for API call writing. 
Zhang et al.~\cite{zhang2024interactive} design a pluggable large languag emodel (LLM) module and retrieval augmented generation (RAG) module to build the knowledge base and contextual memory for decision-making in the brain unit

\subsection{Technical Parts of RAG}
RAG frameworks are based on tripartite foundation, which includes the retrieval, generation and augmentation techniques~\cite{gao2023retrieval}. 

\cite{friel2023chainpoll} apply RAG for LLM hallucination detection. They constructed an RAG-like dataset from COVID-QA
\cite{fatehkia2024t} proposed Tree-RAG (T-RAG) to generate a textual description to augment the context when responding to user queries pertaining to entities within the organization's hierarchy. 

RAG assessment~\cite{es2023ragas}

